FedSDG-FS: Efficient and Secure Feature Selection for Vertical Federated Learning

Vertical Federated Learning (VFL) enables multiple data owners, each holding a different subset of features about largely overlapping sets of data sample(s), to jointly train a useful global model. Feature selection (FS) is important to VFL. It is still an open research problem as existing FS works designed for VFL either assumes prior knowledge on the number of noisy features or prior knowledge on the post-training threshold of useful features to be selected, making them unsuitable for practical applications. To bridge this gap, we propose the Federated Stochastic Dual-Gate based Feature Selection (FedSDG-FS) approach. It consists of a Gaussian stochastic dual-gate to efficiently approximate the probability of a feature being selected, with privacy protection through Partially Homomorphic Encryption without a trusted third-party. To reduce overhead, we propose a feature importance initialization method based on Gini impurity, which can accomplish its goals with only two parameter transmissions between the server and the clients. Extensive experiments on both synthetic and real-world datasets show that FedSDG-FS significantly outperforms existing approaches in terms of achieving accurate selection of high-quality features as well as building global models with improved performance.

==> overview.tex <==
\subsection{Problem Formulations}
There are two entities involved in FL: a cloud server $S$ and $K$ distributed clients  $\{1, 2, \cdots, K\}$. 
% $K$ could be a large number.
Each client $k$ possesses a local dataset $\mathcal{D}_k$.  
%Clients' local datasets are $\mathbb{D}=\{\mathcal{D}_1, \mathcal{D}_2, \dots, \mathcal{D}_K \}$, where  $\mathcal{D}_i$ is the local dataset of $\mathcal{C}_i$.
Under the coordination of the server, all clients collaboratively train a global model $\theta^*\in \mathbb{R}^d$ by sharing their local models updated by their private dataset. Our goal is to construct FL models with high accuracy-to-time performances  considering a very likely situation in real-world where some clients may possess biased training datasets, e.g., data heterogeneity and data noises, which would result in slow convergence speed and low prediction accuracy. Specifically, we can divide all local samples into qualified samples, and negatively influential samples, by their effects to the objective of the global model.
A desired FL framework should enable all participants to collaboratively select important samples for participating model training, while solving training set bias problems by eliminating negatively influential samples. 
The goal of sample selection in FL is to dynamically select a subset of clients and their individual samples, and construct a global model $\theta^*$ based on the selected clients and samples.
The selection of samples and clients, and choice of global parameters can be evaluated by minimizing the following risk:
% dynamically
\begin{equation}
\label{eq:fl-selection-goal}
\begin{split}
    \theta^*(P, p)=\arg\min_{\theta} \mathbb{E}_{k\sim P_k}\mathbb{E}_{z_{k,i}\sim p_{k,i}} [l_{k,i}(\theta)],
\end{split}
\end{equation}
where $0\leq P_k, p_{k,i}\leq 1, k\in [K]$ are the probabilities that client $k$ and the $i$-th sample of client $k$ are selected.
We assume that all participants including the server are semi-honest, \emph{i.e.}, they follow the exact protocol of FL and selection but may be curious about others’ local data. 
% quickly train a global model with a small number of selected important samples, while not putting resources on those  non-important and negatively influential samples. 
\subsection{Design Goals}
We aim to design an FL framework supporting collaborative sample selection and model updating to achieve the following objectives:
\begin{itemize}
    \item \textbf{Effective selection:} the framework should accurately select important clients and their individual important samples that have large positive effects to the objective of the global model, and filter negatively influential clients and samples out from training. Based on the selection results, the framework should further improve the model performance in terms of convergence speed and inference accuracy.
    \item \textbf{Privacy preserving:}
    the framework should preserve each client’s data privacy, that is the local training data should not be exposed to any other party, including the server, during the selection and updating process.
    \item \textbf{Low extra cost:} considering the resource constraints of edge and mobile devices, the selection process should not cause high extra computation and communication cost for clients.
    
\end{itemize}

\subsection{Sample and Client Selection for FL via Meta-Learning}
In the presence of training set biases in FL, to achieve accurate client selection and sample selection while simultaneously training the global model in FL, we need to dynamically quantify the influences of clients and samples on the global model during training, and increase the probability of selection for highly influential clients and its corresponding highly influential samples.
To achieve this, we derive our model from a meta-learning objective towards an online approximation.
Specifically, assume that there is a small amount of unbiased and clean validation set $\{z_i^v=(x_i^v, y_i^v)\in \mathcal{X}\times \mathcal{Y}\}, i\in [M]$, and $M \ll N$, stored at the server. This assumption is reasonable in practical FL scenarios, for instance, Google enlists its employees to type with Gboard to create the root dataset for its federated next-word prediction \cite{GoogleAI}; or the service provider can hire human workers to label some digits for digit recognition task. 
Then the objective in Eq. \eqref{eq:fl-selection-goal} can be re-expressed into the following
\begin{equation}
\label{eq:goal-train}
    \begin{split}
        \theta^*(P, p)&=\arg\min_{\theta}  \sum_{k=1}^{K}\frac{n_k}{n}P_k L_k(\theta), \\
    {\rm where} 
	\,  &L_k(\theta) =\frac{1}{n_k}\sum_{i=1}^{n_k}p_{k,i} l_{k,i}(\theta),
    \end{split}
\end{equation}
with $P, p$ unknown at beginning, where the optimal selection of $P, p$ are calculated based on the performance of the validation set with the objective, 
\begin{equation}
\label{eq:goal-validate}
\begin{split}
    P^*, p^*=\arg \min_{P, p} \frac{1}{M} \sum_{i=1}^M l_i^v(\theta^*(P, p)),
\end{split}
\end{equation}
where $l_i^v(\cdot)$ is the loss function of the validation sample $z_i^v$. 


Calculating the optimal $P^*, p^*$ and $\theta^*$ require two nested loops of optimization, and each single loop can be computational prohibitive. 
% However, since each local sample need to be selected to calculate and transmit $(\frac{1}{K}\sum_{i=1}^{K}H_k)^{-1}\nabla_{\theta}l_i^v(\theta_t(P, p))$ in each iteration, this would  be still much communication-intensive. 
% non-convex targets of FL, the hvp method is not quality guaranteed. and there is no quality guarantee of the approximation for the non-convex problems. However, the objectives in FL are typically non-convex, are not directly applicable in the FL setting. 
Meanwhile, compared with the traditional FL setting defined in Eq. \eqref{eq:optimization-FL}, the outer-loop optimization causes additional computation, which slows down the convergence of the global model, and incurs significant computation and communication overhead, especially for large-scale FL systems. In addition, calculating the optimal $P^*, p^*$ require access to all local training samples or training process. However, in FL systems, the training data and training process are obfuscated from any third party including the server. 

To address the above challenges, we adopt an online strategy to jointly update $P, p$ and $\theta$, respectively, through a single optimization loop to guarantee the efficiency of the algorithm.
The optimization loop is conducted in an iterative way, where we calculate $\theta^*(P, p)$ based on a given $P, p$, then we update $P, p$ based on the obtained $\theta^*(P, p)$. For each training iteration, we determine the probability of a sample being selected based on both the decent direction of some training samples on the training loss surface, and the similarity to the decent direction of the validation loss surface. 



